Revisiting and Exploring Efficient Fast Adversarial Training via LAW: Lipschitz Regularization and Auto Weight Averaging

Fast Adversarial Training (FAT) not only improves the model robustness but also reduces the training cost of standard adversarial training. However, fast adversarial training often suffers from Catastrophic Overfitting (CO), which results in poor robustness performance. Catastrophic Overfitting describes the phenomenon of a sudden and significant decrease in robust accuracy during the training of fast adversarial training. Many effective techniques have been developed to prevent Catastrophic Overfitting and improve the model robustness from different perspectives. However, these techniques adopt inconsistent training settings and require different training costs, i.e, training time and memory costs, leading to unfair comparisons. In this paper, we conduct a comprehensive study of over 10 fast adversarial training methods in terms of adversarial robustness and training costs. We revisit the effectiveness and efficiency of fast adversarial training techniques in preventing Catastrophic Overfitting from the perspective of model local nonlinearity and propose an effective Lipschitz regularization method for fast adversarial training. Furthermore, we explore the effect of data augmentation and weight averaging in fast adversarial training and propose a simple yet effective auto weight averaging method to improve robustness further. By assembling these techniques, we propose a FGSM-based fast adversarial training method equipped with Lipschitz regularization and Auto Weight averaging, abbreviated as FGSM-LAW. Experimental evaluations on four benchmark databases demonstrate the superiority of the proposed method over state-of-the-art fast adversarial training methods and the advanced standard adversarial training methods.

==> Fig/Fig_Initialization.tex <==
\begin{figure*}[t]
\begin{center}
   \includegraphics[width=1\linewidth]{Images/Fig_Initialization.pdf}
\end{center}
\vspace{-3mm}
\caption{The PGD-10 accuracy of fast adversarial training methods with different initialization of different step sizes on the CIFAR10 testing database during the training phase.
% The strategy network is trained using REINFORCE gradients. 
%some non-differentiable operations (\emph{e.g.} choosing the iteration times) related to attack break gradient flow from the target network to the strategy network. As an alternative approach, REINFORCE algorithm~\cite{williams1992simple} is applied to optimize the strategy network and we utilize the so-called ``REINFORCE gradient" to update the strategy network.
}
% The target network provides feedbacks to update the strategy network. }
\label{fig:Fig_Initialization}
\vspace{-3mm}
\end{figure*}

==> Fig/Fig_aug.tex <==
\begin{figure*}[t]
\begin{center}
   \includegraphics[width=0.95\linewidth]{Images/aug_v4.pdf}
\end{center}
\vspace{-6mm}
\caption{The performance of FAT methods with different data augmentation methods on CIFAR10 during the training phase. 
(a): The clean accuracy on the clean images. 
(b): The robustness accuracy under PGD-10. (c): The attack success rate on the AEs used for training.}
% The target network provides feedbacks to update the strategy network. }
\label{fig:aug}
\vspace{-4mm}
\end{figure*}

==> latex/proof.tex <==
Actually the proposed regularization corresponds to a new sample-based local linearity metric of loss function $\ell$ corresponding to $(\mathbf{x},\mathbf{y})$ and $\boldsymbol{\delta}$:
\begin{equation}
\mathbb{E}_{\boldsymbol{\eta}}\left[\frac{\left|f(\mathbf{x}+\boldsymbol{\delta} ; \boldsymbol{\theta})-f(\mathbf{x}+\boldsymbol{\eta} ; \boldsymbol{\theta})\right|}{\|\boldsymbol{\delta}-\boldsymbol{\eta}\|_2}\textbf{}\right].
\end{equation}
This metric is bounded with the gradient of $f$ at $(\mathbf{x}+\boldsymbol{\delta},\mathbf{y})$ as
\begin{equation}
    \begin{aligned}
    & & &\ \ \mathbb{E}_{\boldsymbol{\eta}}\left[\frac{\left|f(\mathbf{x}+\boldsymbol{\delta} ; \boldsymbol{\theta})-f(\mathbf{x}+\boldsymbol{\eta} ; \boldsymbol{\theta})\right|}{\|\boldsymbol{\delta}-\boldsymbol{\eta}\|_2}\textbf{}\right]\\[3pt]
    & &\leq&\ \ \mathbb{E}_{\boldsymbol{\eta}}\left[\frac{|\nabla^{\top}_{\mathbf{x}}f(\mathbf{x}+\boldsymbol{\delta};\boldsymbol{\theta})(\boldsymbol{\delta}-\boldsymbol{\eta})|}{\|\boldsymbol{\delta}-\boldsymbol{\eta}\|_2}\right]\\[3pt]
    & &\leq&\ \ \mathbb{E}_{\boldsymbol{\eta}}\left[\frac{\|\nabla_{\mathbf{x}}f(\mathbf{x}+\boldsymbol{\delta};\boldsymbol{\theta})\|_2\|\boldsymbol{\delta}-\boldsymbol{\eta}\|_2}{\|\boldsymbol{\delta}-\boldsymbol{\eta}\|_2}\right]\\[5pt]
    & &\leq&\ \  \|\nabla_{\mathbf{x}}f(\mathbf{x}+\boldsymbol{\delta};\boldsymbol{\theta})\|_2\leq\underset{\mathbf{x}}{\textbf{max}} \|\nabla_{\mathbf{x}}f(\mathbf{x};\boldsymbol{\theta})\|_2.
    \end{aligned}
\end{equation}
The first inequality holds as the score function $f(\cdot,\cdot)$ is a convex function \textit{w.r.t} $\mathbf{x}$ and the second one holds by the H\"{o}lder inequality. It means that the proposed metric is bounded by the gradient of the adversarial perturbation $(\mathbf{x}+\boldsymbol{\delta}, \mathbf{y})$. Then it could generate the parsimonious effect on the local Lipschitzness for any $(\mathbf{x},\mathbf{y})\sim\mathcal{D}$. As a consequence, the proposed regularization could produce a more robust model than the existing adversarial training methods.

==> table/HP_WA.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using ResNet18 equipped with auto weight averaging with diffrerent hyper-parameters $\Delta$. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
 }
\label{table:HP_WA}
\scalebox{0.92}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
\toprule
Hyper-Parameter & Clean & PGD-10         & PGD-20        & PGD-50         & C\&W           & AA             & Time \\ \midrule
Baseline    & \textbf{86.82} & 46.62  & 44.76  & 44.23  & 45.89 & 42.37  & 1 $\times$    \\ \midrule \midrule
$\Delta=0.6$    & 79.98 & 51.47 & \textbf{50.7} & \textbf{50.53} & 48.53          & 46.08          & 1 $\times$   \\ \midrule
$\Delta=0.65$   & 80.92 & \textbf{51.69}          & 50.9          & 49.73          & 49.15          & 46.18          & 1 $\times$   \\ \midrule
$\Delta=0.7$    & 81.82 & 50.94          & 50.11         & 49.85          & 49.21          & 46.22          & 1 $\times$    \\ \midrule
$\Delta=0.75$   & 83.62 & 51.26          & 50.21         & 49.9           & \textbf{49.42} & \textbf{46.53} & 1 $\times$   \\ \midrule
$\Delta=0.8$    & 85.76 & 48.9           & 47.35         & 46.89          & 47.59          & 44.33          & 1 $\times$   \\ \midrule
$\Delta=0.85$   & 86.7  & 47.83          & 46.04         & 45.68          & 46.84          & 43.47          & 1 $\times$   \\ \bottomrule
\end{tabular}
}
\end{table}


==> table/HP_WA_v1.tex <==
\begin{table}[h]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using ResNet18 equipped with auto weight averaging with diffrerent hyper-parameters $\Delta$. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
 }
\label{table:HP_WA}
\scalebox{0.75}{
\begin{tabular}{cccccccc}
\toprule
Hyper-Parameter & Clean & PGD-10         & PGD-20        & PGD-50         & C\&W           & AA             & \begin{tabular}[c]{@{}c@{}}Training\\ Time (min)\end{tabular} \\ \midrule
Baseline    & \textbf{86.82} & 46.62  & 44.76  & 44.23  & 45.89 & 42.37  & 51    \\ \midrule \midrule
$\Delta=0.6$    & 79.98 & 51.47 & \textbf{50.7} & \textbf{50.53} & 48.53          & 46.08          & 52   \\ \midrule
$\Delta=0.65$   & 80.92 & \textbf{51.69}          & 50.9          & 49.73          & 49.15          & 46.18          & 52   \\ \midrule
$\Delta=0.7$    & 81.82 & 50.94          & 50.11         & 49.85          & 49.21          & 46.22          & 52    \\ \midrule
$\Delta=0.75$   & 83.62 & 51.26          & 50.21         & 49.9           & \textbf{49.42} & \textbf{46.53} & 52   \\ \midrule
$\Delta=0.8$    & 85.76 & 48.9           & 47.35         & 46.89          & 47.59          & 44.33          & 52   \\ \midrule
$\Delta=0.85$   & 86.7  & 47.83          & 46.04         & 45.68          & 46.84          & 43.47          & 52   \\ \bottomrule
\end{tabular}
}
\end{table}


==> table/HP_regular.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using ResNet18 with equipped with Lipschitz regularization with different hyper-parameter $\lambda$ . Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
 }
\label{table:HP_regular}
\scalebox{0.92}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
\toprule
 Hyper-Parameter & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W           & AA             & Time \\ \midrule
Baseline    & \textbf{86.82} & 46.62  & 44.76  & 44.23  & 45.89 & 42.37  & 1 $\times$    \\ \midrule \midrule
$\lambda=8$      & 84.34 & 54.09          & 53.21          & 52.88          & 49.28          & 46.57          & 1.4 $\times$ \\ \midrule
$\lambda=10$     & 84.04          & 84.04          & 54.31          & 53.03          & 49.83          & 47.08          & 1.4 $\times$ \\ \midrule
$\lambda=12$     & 83.35          & 53.94          & 54.03          & 53.66          & 50.05          & 47.38          & 1.4 $\times$ \\ \midrule
$\lambda=14$    & 82.97          & \textbf{55.49} & \textbf{54.58} & \textbf{54.29} & \textbf{50.41} & \textbf{48.05} & 1.4 $\times$ \\ \midrule
$\lambda=16$     & 83.49          & 54.86          & 53.99          & 53.62          & 49.53          & 47.11          & 1.4 $\times$  \\ \midrule
$\lambda=18$     & 82.74          & 55.2           & 54.35          & 54.27          & 50.17          & 47.58          & 1.4 $\times$  \\ \bottomrule
\end{tabular}
}
\end{table}


==> table/HP_regular_v1.tex <==
\begin{table}[h]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using ResNet18 with equipped with Lipschitz regularization with different hyper-parameter $\lambda$ . Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
 }
\label{table:HP_regular}
\scalebox{0.75}{
\begin{tabular}{cccccccc}
\toprule
 Hyper-Parameter & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W           & AA             & \begin{tabular}[c]{@{}c@{}}Training\\ Time (min)\end{tabular}  \\ \midrule
Baseline    & \textbf{86.82} & 46.62  & 44.76  & 44.23  & 45.89 & 42.37  & 51    \\ \midrule \midrule
$\lambda=8$      & 84.34 & 54.09          & 53.21          & 52.88          & 49.28          & 46.57          & 73 \\ \midrule
$\lambda=10$     & 84.04          & 84.04          & 54.31          & 53.03          & 49.83          & 47.08          & 73 \\ \midrule
$\lambda=12$     & 83.35          & 53.94          & 54.03          & 53.66          & 50.05          & 47.38          & 73 \\ \midrule
$\lambda=14$    & 82.97          & \textbf{55.49} & \textbf{54.58} & \textbf{54.29} & \textbf{50.41} & \textbf{48.05} & 73 \\ \midrule
$\lambda=16$     & 83.49          & 54.86          & 53.99          & 53.62          & 49.53          & 47.11          & 73  \\ \midrule
$\lambda=18$     & 82.74          & 55.2           & 54.35          & 54.27          & 50.17          & 47.58          & 73  \\ \bottomrule
\end{tabular}
}
\end{table}


==> table/Tiny_ImageNet.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the Tiny ImageNet database using PreActResNet18 with different adversarial training methods. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:Tiny_ImageNet}
\scalebox{0.82}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
\toprule
Method       & \begin{tabular}[c]{@{}c@{}}Clean\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-10\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-20\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-50\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\&W\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}AA\\ Best/Last\end{tabular} & Time \\ \midrule
PGD-AT       & 43.6/45.28                                                  & 20.2/16.12                                                   & 19.9/15.6                                                    & 19.86/15.4                                                   & 17.5/14.28                                                 & 16.0/12.84                                               & 5.2$\times$   \\ \midrule \midrule
FGSM-RS      & 44.98/45.18                                                 & 17.72/0.00                                                   & 17.46/0.00                                                   & 17.36/0.00                                                   & 15.84/0.00                                                 & 14.08/0.00                                               & 1 $\times$    \\ \midrule
FGSM-PGI     & 43.32/45.88                                                 & 23.8/22.02                                                   & 23.4/21.7                                                    & 23.38/21.6                                                    & 19.28/17.44                                                & \textbf{17.56}/15.50                                              & 1.4 $\times$   \\ \midrule
FGSM-CKPT    & \textbf{49.98/49.98}                                        & 9.20/9.20                                                    & 9.20/9.20                                                    & 8.68/8.68                                                    & 9.24/9.24                                                  & 8.10/8.10                                                & 1.5 $\times$   \\ \midrule
FGSM-SDI     & 46.46/47.64                                                 & 23.22/19.84                                                  & 22.84/19.36                                                  & 22.76/19.16                                                  & 18.54/16.02                                                & 17.0/14.10                                               & 1.6 $\times$   \\ \midrule
NuAT         & 42.9/42.42                                                  & 15.12/13.78                                                  & 14.6/13.34                                                   & 14.44/13.2                                                   & 12.02/11.32                                                & 10.28/9.56                                               & 2.0 $\times$   \\ \midrule
GAT          & 42.16/41.84                                                 & 15.02/14.44                                                  & 14.5/13.98                                                   & 14.44/13.8                                                   & 11.78/11.48                                                & 10.26/9.74                                               & 2.0 $\times$   \\ \midrule
FGSM-GA      & 43.44/43.44                                                 & 18.86/18.86                                                  & 18.44/18.44                                                  & 18.36/18.36                                                  & 16.2/16.2                                                  & 14.28/14.28                                              & 3.5 $\times$   \\ \midrule
Free-AT (m=8) & 38.9/40.06                                                  & 11.62/8.84                                                   & 11.24/8.32                                                   & 11.02/8.2                                                    & 11.00/8.08                                                 & 9.28/7.34                                                & 4.2 $\times$   \\ \midrule
FGSM-LAW (ours)    & 47.74/47.74                                                 & \textbf{24.45/24.45}                                         & \textbf{24.09/24.09}                                         & \textbf{24.06/24.06}                                         & \textbf{18.65/18.65}                                       & 16.43/\textbf{16.43}                                     & 1.4 $\times$ \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/ablation.tex <==
\begin{table}[!htb]
\centering
\caption{ Ablation study on CIFAR-10. Clean and robust accuracy (\%) and training time on the CIFAR-10 database using ResNet18 under $\ell_{\infty}= 8/225$. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:ablation}
\scalebox{0.72}{
\begin{tabular}{cccccccc}
\toprule
L-Regular (Ours) & Cutout & A-WA (Ours) & Clean          & PGD-50         & C\&W             & AA             & \begin{tabular}[c]{@{}c@{}}Training\\ Time (min)\end{tabular} \\ \midrule
                   &        &                      & \textbf{86.82} & 44.23          & 45.89         & 42.37           &     51   \\ \midrule  \midrule 
     \checkmark    &        &                      & 82.97          & 54.29          & 50.41          & 48.05          &    73    \\ \midrule
    \checkmark     &   \checkmark     &                      & 82.55          & 55.08          & 50.69          & 48.63          &     80  \\ \midrule
    \checkmark     &        &       \checkmark               & 80.38          & 56.33          & 51.48          & 49.27          &    74  \\ \midrule
     \checkmark    &   \checkmark     &         \checkmark             & 80.46          & \textbf{56.72} & \textbf{51.76} & \textbf{49.36} &   81   \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/category.tex <==
\begin{table*}[t]
\centering
\caption{ The category result of the existing fast adversarial training methods. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10_implement}

\scalebox{0.6}{
\begin{tabular}{@{}c|cccccccccc@{}}
\toprule
FAT Method     & \multicolumn{1}{c|}{FGSM-AT} & \multicolumn{1}{c|}{FGSM-RS} & \multicolumn{1}{c|}{FGSM-GA}   & \multicolumn{1}{c|}{FGSM-CKPT} & \multicolumn{1}{c|}{NUAT} & \multicolumn{1}{c|}{GAT}      & \multicolumn{1}{c|}{SLAT}    & \multicolumn{1}{c|}{ATTA}     & \multicolumn{1}{c|}{FGSM-PGI} & FGSM-SDI       \\ \midrule
Initialization & \multicolumn{7}{c|}{Random-based}                                                                                                                                                                                        & \multicolumn{2}{c|}{Prior-based}                              & Learning-based \\ \midrule \midrule
FAT Method     & \multicolumn{1}{c|}{FGSM-AT} & \multicolumn{1}{c|}{FGSM-RS} & \multicolumn{1}{c|}{FGSM-CKPT} & \multicolumn{1}{c|}{SLAT}      & \multicolumn{1}{c|}{ATTA} & \multicolumn{1}{c|}{FGSM-SDI} & \multicolumn{1}{c|}{FGSM-GA} & \multicolumn{1}{c|}{FGSM-PGI} & \multicolumn{1}{c|}{NUAT}     & GAT            \\ \midrule
Regularization & \multicolumn{6}{c|}{without Regularization}                                                                                                                                               & \multicolumn{2}{c|}{Minimization Optimization}               & \multicolumn{2}{c}{Min-max Optimization}      \\ \bottomrule
\end{tabular}
}
\end{table*}

==> table/cifar10.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using ResNet18 with different adversarial training methods. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10}
\scalebox{0.92}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c|c|c@{}}
\toprule
Method                        &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W           & AA             & \begin{tabular}[c]{@{}c@{}}Data \\ Memory\end{tabular}                    & Time(min)            \\ \midrule
\multirow{2}{*}{PGD-AT}       & Best & 82.32          & 53.76          & 52.83          & 52.6           & 51.08          & 48.68          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{5.2 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 82.65          & 53.39          & 52.52          & 52.27          & 51.28          & 48.93          &                                                                           &                      \\ \midrule \midrule
\multirow{2}{*}{FGSM-RS}      & Best & 73.81          & 42.31          & 41.55          & 41.26          & 39.84          & 37.07          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{1 $\times$}   \\ \cmidrule(lr){2-8}
                              & Last & 83.82          & 00.09          & 00.04          & 00.02          & 0.00           & 0.00           &                                                                           &                      \\ \midrule
\multirow{2}{*}{FGSM-PGI}     & Best & 81.72          & 55.18          & 54.36          & 54.17          & 50.75          & 49.00          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Whole \\ Dataset\end{tabular}} & \multirow{2}{*}{1.4 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 81.72          & 55.18          & 54.36          & 54.17          & 50.75          & 49.00          &                                                                           &                      \\ \midrule
\multirow{2}{*}{FGSM-CKPT}    & Best & \textbf{90.29} & 41.96          & 39.84          & 39.15          & 41.13          & 37.15          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{1.5 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & \textbf{90.29} & 41.96          & 39.84          & 39.15          & 41.13          & 37.15          &                                                                           &                      \\ \midrule
\multirow{2}{*}{FGSM-SDI}     & Best & 84.86          & 53.73          & 52.54          & 52.18          & 51.00          & 48.50          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{1.6 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 85.25          & 53.18          & 52.05          & 51.79          & 50.29          & 47.91          &                                                                           &                      \\ \midrule
\multirow{2}{*}{NuAT}         & Best & 81.58          & 53.96          & 52.9           & 52.61          & 51.3           & 49.09          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{2.0 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 81.38          & 53.52          & 52.65          & 52.48          & 50.63          & 48.70          &                                                                           &                      \\ \midrule
\multirow{2}{*}{GAT}          & Best & 79.79          & 54.18          & 53.55          & 53.42          & 49.04          & 47.53          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{2.0 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 80.41          & 53.29          & 52.06          & 51.76          & 49.07          & 46.56          &                                                                           &                      \\ \midrule
\multirow{2}{*}{FGSM-GA}      & Best & 83.96          & 49.23          & 47.57          & 46.89          & 47.46          & 43.45          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{3.5 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 84.43          & 48.67          & 46.66          & 46.08          & 46.75          & 42.63          &                                                                           &                      \\ \midrule
\multirow{2}{*}{Free-AT(m=8)} & Best & 80.38          & 47.1           & 45.85          & 45.62          & 44.42          & 42.17          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{4.2 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 80.75          & 45.82          & 44.82          & 44.48          & 43.73          & 41.17          &                                                                           &                      \\ \midrule
\multirow{2}{*}{Ours}         & Best & 80.46          & \textbf{57.33} & \textbf{56.83} & \textbf{56.72} & \textbf{51.76} & \textbf{49.36} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{1.4 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 80.46          & \textbf{57.33} & \textbf{56.83} & \textbf{56.72} & \textbf{51.76} & \textbf{49.36} &                                                                           &                      \\ \bottomrule
\end{tabular}
}
\end{table}
 

==> table/cifar100.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-100 database using ResNet18 with different adversarial training methods. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar100}
\scalebox{0.92}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c|c|c@{}}
\toprule
Method                        &      & Clean          & PGD-10         & PGD-20         & PGD-50         & C\&W           & AA             & \begin{tabular}[c]{@{}c@{}}Data \\ Memory\end{tabular}                    & Time(min)            \\ \midrule
\multirow{2}{*}{PGD-AT}       & Best & 57.52          & 29.6           & \textbf{28.99}          & 28.87          & 28.85          & 25.48          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{5.2 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 57.5           & 29.54          & 29.00          & 28.90          & 27.6           & 25.58          &                                                                           &                      \\ \midrule \midrule
\multirow{2}{*}{FGSM-RS}      & Best & 49.85          & 22.47          & 22.01          & 21.82          & 20.55          & 18.29          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{1 $\times$}   \\ \cmidrule(lr){2-8}
                              & Last & 60.55          & 00.45          & 00.25          & 00.19          & 00.25          & 0.00           &                                                                           &                      \\ \midrule
\multirow{2}{*}{FGSM-PGI}     & Best & 58.78          & 31.88          & 31.26          & 31.14          & 28.06          & 25.67          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Whole \\ Dataset\end{tabular}} & \multirow{2}{*}{1.4 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 58.81 & 31.6           & 31.06          & 30.88          & 27.72          & 25.42          &                                                                           &                      \\ \midrule
\multirow{2}{*}{FGSM-CKPT}    & Best & \textbf{60.93} & 16.58          & 15.47          & 15.19          & 16.4           & 14.17          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{1.5 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & \textbf{60.93} & 16.69          & 15.61          & 15.24          & 16.6           & 14.34          &                                                                           &                      \\ \midrule
\multirow{2}{*}{FGSM-SDI}     & Best & 60.67          & 31.5           & 30.89          & 30.6           & 27.15          & 25.23          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{1.6 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 60.82          & 30.87          & 30.34          & 30.08          & 27.3           & 25.19          &                                                                           &                      \\ \midrule
\multirow{2}{*}{NuAT}         & Best & 59.71          & 27.54          & 23.02          & 20.18          & 22.07          & 11.32          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{2.0 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 59.62          & 27.07          & 22.72          & 20.09          & 21.59          & 11.55          &                                                                           &                      \\ \midrule
\multirow{2}{*}{GAT}          & Best & 57.01          & 24.55          & 23.8           & 23.55          & 22.02          & 19.60          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{2.0 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 56.07          & 23.92          & 23.18          & 23.0           & 21.93          & 19.51          &                                                                           &                      \\ \midrule
\multirow{2}{*}{FGSM-GA}      & Best & 54.35          & 22.93          & 22.36          & 22.2           & 21.2           & 18.88          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{3.5 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 55.1           & 20.04          & 19.13          & 18.84          & 18.96          & 16.45          &                                                                           &                      \\ \midrule
\multirow{2}{*}{Free-AT(m=8)} & Best & 52.49          & 24.07          & 23.52          & 23.36          & 21.66          & 19.47          & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{4.2 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 52.63          & 22.86          & 22.32          & 22.16          & 20.68          & 18.57          &                                                                           &                      \\ \midrule
\multirow{2}{*}{Ours}         & Best & 58.79          & \textbf{31.8} & \textbf{31.35} & \textbf{31.33} & \textbf{28.47} & \textbf{25.78} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}}     & \multirow{2}{*}{1.4 $\times$} \\ \cmidrule(lr){2-8}
                              & Last & 58.79          & \textbf{31.8} & \textbf{31.35} & \textbf{31.33} & \textbf{28.47} & \textbf{25.78} &                                                                           &                      \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/cifar100_v2.tex <==
\begin{table*}[!htb]
\centering
\caption{ Test robustness (\%) on the CIFAR-100 database. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar100}
\scalebox{0.85}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
\toprule
Method           & \begin{tabular}[c]{@{}c@{}}Clean\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-10\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-20\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-50\\  Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\&W\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}AA\\  Best/Last\end{tabular} & Time \\ \midrule
PGD-AT           & 57.52/57.5                                                & 29.6/29.54                                                 & 28.99/29.0                                                 & 28.87/28.9                                                  & 28.85/27.6                                               & 25.48/25.58                                             & 5.2 $\times$ \\ \midrule \midrule
FGSM-RS          & 49.85/60.55                                               & 22.47/0.45                                                 & 22.01/0.25                                                 & 21.82/0.19                                                  & 20.55/0.25                                               & 18.29/0.00                                              & 1 $\times$   \\ \midrule
FGSM-PGI         & 58.78/58.81                                               & 31.78/31.6                                                 & 31.26/31.06                                                & 31.14/30.88                                                 & 28.06/27.72                                              & 25.67/25.42                                             & 1.4 $\times$  \\ \midrule
FGSM-CKPT        & \textbf{60.93/60.93}                                      & 16.58/16.69                                                & 15.47/15.61                                                & 15.19/15.24                                                 & 16.4/16.6                                                & 14.17/14.34                                             & 1.5 $\times$  \\ \midrule
FGSM-SDI         & 60.67/60.82                                               & 31.5/30.87                                                 & 30.89/30.34                                                & 30.6/30.08                                                  & 27.15/27.3                                               & 25.23/25.19                                             & 1.6 $\times$  \\ \midrule
NuAT             & 59.71/59.62                                               & 27.54/27.07                                                & 23.02/22.72                                                & 20.18/20.09                                                 & 22.07/21.59                                              & 11.32/11.55                                             & 2.0 $\times$  \\ \midrule
GAT              & 57.01/56.07                                               & 24.55/23.92                                                & 23.8/23.18                                                 & 23.55/23.0                                                  & 22.02/21.93                                              & 19.60/19.51                                             & 2.0 $\times$  \\ \midrule
FGSM-GA          & 54.35/55.1                                                & 22.93/20.04                                                & 22.36/19.13                                                & 22.2/18.84                                                  & 21.2/18.96                                               & 18.88/16.45                                             & 3.5 $\times$  \\ \midrule
Free-AT (m=8)    & 52.49/52.63                                               & 24.07/22.86                                                & 23.52/22.32                                                & 23.36/22.16                                                 & 21.66/20.68                                              & 19.47/18.57                                             & 4.2 $\times$  \\ \midrule
FGSM-LAW (ours) & 58.79/58.79                                               & \textbf{31.8/31.8}                                         & \textbf{31.35/31.35}                                       & \textbf{31.33/31.33}                                        & \textbf{28.47/28.47}                                     & \textbf{25.78/25.78}                                    & 1.4 $\times$  \\ \bottomrule
\end{tabular}
}
\end{table*}

==> table/cifar10_v2.tex <==
\begin{table*}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10}
\scalebox{0.85}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
\toprule
Method           & \begin{tabular}[c]{@{}c@{}}Clean\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-10\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-20\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-50\\  Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\&W\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}AA\\  Best/Last\end{tabular} & Time \\ \midrule
PGD-AT           & 82.32/82.65                                               & 53.76/53.39                                                & 52.83/52.52                                                & 52.6/52.27                                                  & 51.08/51.28                                              & 48.68/48.93                                             & 5.2 $\times$  \\ \midrule \midrule
FGSM-RS          & 73.81/83.82                                               & 42.31/0.09                                                 & 41.55/0.04                                                 & 41.26/0.02                                                  & 39.84/0.00                                               & 37.07/0.00                                              & 1 $\times$   \\ \midrule
FGSM-PGI         & 81.72/81.72                                               & 55.18/55.18                                                & 54.36/54.36                                                & 54.17/54.17                                                 & 50.75/50.75                                              & 49.0/49.0                                               & 1.4 $\times$  \\ \midrule
FGSM-CKPT        & \textbf{90.29/90.29}                                      & 41.96/41.96                                                & 39.84/39.84                                                & 39.15/39.15                                                 & 41.13/41.13                                              & 37.15/37.15                                             & 1.5 $\times$  \\ \midrule
FGSM-SDI         & 84.86/85.25                                               & 53.73/53.18                                                & 52.54/52.05                                                & 52.18/51.79                                                 & 51.0/50.29                                               & 48.50/47.91                                             & 1.6 $\times$  \\ \midrule
NuAT             & 81.58/81.38                                               & 53.96/53.52                                                & 52.9/52.65                                                 & 52.61/52.48                                                 & 51/3/50.63                                               & 49.09/48.70                                             & 2.0 $\times$ \\ \midrule
GAT              & 79.79/80.41                                               & 54.18/53.29                                                & 53.55/52.06                                                & 53.42/51.76                                                 & 49.04/49.07                                              & 47.53/46.56                                             & 2.0 $\times$ \\ \midrule
FGSM-GA          & 83.96/84.43                                               & 49.23/48.67                                                & 47.57/46.66                                                & 46.89/46.08                                                 & 47.46/46.75                                              & 43.45/42.63                                             & 3.5 $\times$ \\ \midrule
Free-AT (m=8)    & 80.38/80.75                                               & 47.1/45.82                                                 & 45.85/44.82                                                & 45.62/44.48                                                 & 44.42/43.73                                              & 42.17/41.17                                             & 4.2 $\times$ \\ \midrule
FGSM-LAW (ours) & 80.46/80.46                                               & \textbf{57.33/57.33}                                       & \textbf{56.83/56.83}                                       & \textbf{56.72/56.72}                                        & \textbf{51.76/51.76}                                     & \textbf{49.36/49.36}                                    & 1.4 $\times$  \\ \bottomrule
\end{tabular}
}
\end{table*}


==> table/experiments.tex <==
\begin{table*}[t]
\centering
\centering
\caption{ Comparisons of clean and robust accuracy (\%) and training time on the CIFAR-10, CIFAR-100 and Tiny ImageNet databases using different adversarial training methods under $\ell_{\infty}= 8/225$. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:experiments}
\scalebox{0.85}{
\begin{tabular}{@{}c|cccc|cccc|cccc|c@{}}
\toprule
Dataset         & \multicolumn{4}{c|}{CIFAR-10}                                                                                                    & \multicolumn{4}{c|}{CIFAR-100}                                                                                                   & \multicolumn{4}{c|}{Tiny ImageNet}                                                                                               & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Training \\ Time\end{tabular}} \\ \cmidrule(r){1-13}
Method          & \multicolumn{1}{c|}{Clean}          & \multicolumn{1}{c|}{PGD-50}         & \multicolumn{1}{c|}{C\&W}           & AA             & \multicolumn{1}{c|}{Clean}          & \multicolumn{1}{c|}{PGD-50}         & \multicolumn{1}{c|}{C\&W}           & AA             & \multicolumn{1}{c|}{Clean}          & \multicolumn{1}{c|}{PGD-50}         & \multicolumn{1}{c|}{C\&W}           & AA             &                                                                           \\ \midrule
PGD-AT          & \multicolumn{1}{c|}{82.65}          & \multicolumn{1}{c|}{52.27}          & \multicolumn{1}{c|}{51.28}          & 48.93          & \multicolumn{1}{c|}{57.5}           & \multicolumn{1}{c|}{28.9}           & \multicolumn{1}{c|}{27.6}           & 25.58          & \multicolumn{1}{c|}{45.28}          & \multicolumn{1}{c|}{15.4}           & \multicolumn{1}{c|}{14.28}          & 12.84          & 5.2×                                                                      \\ \midrule \midrule
FGSM-RS         & \multicolumn{1}{c|}{83.82}          & \multicolumn{1}{c|}{0.02}           & \multicolumn{1}{c|}{0.00}           & 0.00           & \multicolumn{1}{c|}{60.55}          & \multicolumn{1}{c|}{0.19}           & \multicolumn{1}{c|}{0.25}           & 0.00           & \multicolumn{1}{c|}{45.18}          & \multicolumn{1}{c|}{0.00}           & \multicolumn{1}{c|}{0.00}           & 0.00           & 1 ×                                                                       \\ \midrule
FGSM-PGI        & \multicolumn{1}{c|}{81.72}          & \multicolumn{1}{c|}{54.17}          & \multicolumn{1}{c|}{50.75}          & 49.0           & \multicolumn{1}{c|}{58.81}          & \multicolumn{1}{c|}{30.88}          & \multicolumn{1}{c|}{27.72}          & 25.42          & \multicolumn{1}{c|}{45.88}          & \multicolumn{1}{c|}{21.6}           & \multicolumn{1}{c|}{17.44}          & 15.50          & 1.4 ×                                                                     \\ \midrule
FGSM-CKPT       & \multicolumn{1}{c|}{\textbf{90.29}} & \multicolumn{1}{c|}{39.15}          & \multicolumn{1}{c|}{41.13}          & 37.15          & \multicolumn{1}{c|}{\textbf{60.93}} & \multicolumn{1}{c|}{15.24}          & \multicolumn{1}{c|}{16.6}           & 14.34          & \multicolumn{1}{c|}{\textbf{49.98}} & \multicolumn{1}{c|}{8.68}           & \multicolumn{1}{c|}{9.24}           & 8.10           & 1.5 ×                                                                     \\ \midrule
FGSM-SDI        & \multicolumn{1}{c|}{85.25}          & \multicolumn{1}{c|}{51.79}          & \multicolumn{1}{c|}{50.29}          & 47.91          & \multicolumn{1}{c|}{60.82}          & \multicolumn{1}{c|}{30.08}          & \multicolumn{1}{c|}{27.3}           & 25.19          & \multicolumn{1}{c|}{47.64}          & \multicolumn{1}{c|}{19.16}          & \multicolumn{1}{c|}{16.02}          & 14.10          & 1.6 ×                                                                     \\ \midrule
NuAT \tablefootnote{For a fair comparison, we adopt the standard ResNet18 to conduct experiments, but the original NuAT adopts ResNet18 with extra the ReLU layer at each block from the code they provide.}            & \multicolumn{1}{c|}{82.48}          & \multicolumn{1}{c|}{51.02}          & \multicolumn{1}{c|}{50.08}          & 46.89          & \multicolumn{1}{c|}{59.62}          & \multicolumn{1}{c|}{20.09}          & \multicolumn{1}{c|}{21.59}          & 11.55          & \multicolumn{1}{c|}{42.42}          & \multicolumn{1}{c|}{13.2}           & \multicolumn{1}{c|}{11.32}          & 9.56           & 2.0 ×                                                                     \\ \midrule
GAT             & \multicolumn{1}{c|}{80.41}          & \multicolumn{1}{c|}{51.76}          & \multicolumn{1}{c|}{49.07}          & 46.56          & \multicolumn{1}{c|}{56.07}          & \multicolumn{1}{c|}{23.0}           & \multicolumn{1}{c|}{21.93}          & 19.51          & \multicolumn{1}{c|}{41.84}          & \multicolumn{1}{c|}{13.8}           & \multicolumn{1}{c|}{11.48}          & 9.74           & 2.0 ×                                                                     \\ \midrule
FGSM-GA         & \multicolumn{1}{c|}{84.43}          & \multicolumn{1}{c|}{46.08}          & \multicolumn{1}{c|}{46.75}          & 42.63          & \multicolumn{1}{c|}{55.1}           & \multicolumn{1}{c|}{18.84}          & \multicolumn{1}{c|}{18.96}          & 16.45          & \multicolumn{1}{c|}{43.44}          & \multicolumn{1}{c|}{18.36}          & \multicolumn{1}{c|}{16.2}           & 14.28          & 3.5 ×                                                                     \\ \midrule
Free-AT (m=8)   & \multicolumn{1}{c|}{80.75}          & \multicolumn{1}{c|}{44.48}          & \multicolumn{1}{c|}{43.73}          & 41.17          & \multicolumn{1}{c|}{52.63}          & \multicolumn{1}{c|}{22.16}          & \multicolumn{1}{c|}{20.68}          & 18.57          & \multicolumn{1}{c|}{40.06}          & \multicolumn{1}{c|}{8.2}            & \multicolumn{1}{c|}{8.08}           & 7.34           & 4.2 ×                                                                     \\ \midrule
FGSM-LAW (ours) & \multicolumn{1}{c|}{80.46}          & \multicolumn{1}{c|}{\textbf{56.72}} & \multicolumn{1}{c|}{\textbf{51.76}} & \textbf{49.36} & \multicolumn{1}{c|}{58.79}          & \multicolumn{1}{c|}{\textbf{31.33}} & \multicolumn{1}{c|}{\textbf{28.47}} & \textbf{25.78} & \multicolumn{1}{c|}{47.74}          & \multicolumn{1}{c|}{\textbf{24.06}} & \multicolumn{1}{c|}{\textbf{18.65}} & \textbf{16.43} & 1.4 ×                                                                     \\ \bottomrule
\end{tabular}
}
\end{table*}
 

==> table/implement.tex <==
\begin{table*}[t]
\centering
\caption{ The techniques used in different fast adversarial training methods on CIFAR-10. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10_implement}

\scalebox{0.82}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c|c@{}}
\toprule
  Method        & Initialization & \begin{tabular}[c]{@{}c@{}}Step \\ Size\end{tabular} & Regularization & \begin{tabular}[c]{@{}c@{}}Training \\ Time\end{tabular} & \begin{tabular}[c]{@{}c@{}}Data \\ Memory \end{tabular} & \begin{tabular}[c]{@{}c@{}}Early \\ Stop\end{tabular} & \begin{tabular}[c]{@{}c@{}}CO w/o \\ Early Stop\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textgreater 45\% \\ under AA\end{tabular} \\ \midrule \midrule
FGSM-AT   &      $\eta = 0 $       & $\epsilon$         & \usym{2717}             & 1 $\times$   &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}       & \usym{2714}        & \usym{2714}               & \usym{2717}                         \\ \midrule
Free-AT   &        $\eta = 0 $        & $\epsilon$          & \usym{2717}             & 4.2 $\times$  &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}        & \usym{2717}         & \usym{2717}                & \usym{2717}                         \\ \midrule
FGSM-RS   &     $\eta \in \mathbf{U}(-\epsilon, \epsilon)$           & 1.25$\epsilon$       & \usym{2717}             & 1 $\times$   &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}          & \usym{2714}        & \usym{2714}               & \usym{2717}                         \\ \midrule
FGSM-GA   &     $\eta \in \mathbf{U}(-\epsilon, \epsilon)$           & 1.25$\epsilon$       & \usym{2714}            & 3.5 $\times$   &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}         & \usym{2714}        & \usym{2717}                & \usym{2717}                         \\ \midrule
FGSM-CKPT &    $\eta \in \mathbf{U}(-\epsilon, \epsilon)$            & 1.25$\epsilon$    & \usym{2717}             & 1.5 $\times$   &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}        & \usym{2717}         & \usym{2717}                & \usym{2717}                         \\ \midrule
ATTA      &    $\eta_{t+1}=\boldsymbol{\delta}_{E} $             & $\epsilon$          & \usym{2717}             & 1 $\times$    &     \begin{tabular}[c]{@{}c@{}}Whole \\ Dataset \end{tabular}         & \usym{2717}         & \usym{2717}                & \usym{2717}                         \\ \midrule
NuAT      &    $\eta \in \mathbf{B}(-\epsilon/2, \epsilon/2)$            & $\epsilon$          & \usym{2714}            & 2 $\times$     &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}         & \usym{2717}         & \usym{2717}                & \usym{2714}                        \\ \midrule
GAT       &   $\eta \in \mathbf{B}(-\epsilon/2, \epsilon/2)$              & $\epsilon$          & \usym{2714}            & 2 $\times$  &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}          & \usym{2717}         & \usym{2717}                & \usym{2714}                        \\ \midrule
SLAT      &      $\eta \in \mathbf{U}(-\epsilon, \epsilon)$          & $\epsilon$          & \usym{2714}            & 1.1 $\times$   &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}         & \usym{2717}         & \usym{2717}                & \usym{2717}                         \\ \midrule
FGSM-SDI  &       $\eta=\epsilon \cdot g\left(,\theta\right)$         & $\epsilon$          & \usym{2717}             & 1.6 $\times$   &     \begin{tabular}[c]{@{}c@{}}One \\ Batch \end{tabular}        & \usym{2717}         & \usym{2717}                & \usym{2714}                        \\ \midrule
FGSM-PGI  &        $\eta_{t+1}=\boldsymbol{\delta}_{P} $       & $\epsilon$         & \usym{2714}            & 1.4 $\times$    &     \begin{tabular}[c]{@{}c@{}}Whole \\ Dataset \end{tabular}       & \usym{2717}         & \usym{2717}                & \usym{2714}                        \\ \bottomrule
\end{tabular}
}
\end{table*}

==> table/init.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using ResNet18 with different sample initialization techniques. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10_init}
\scalebox{0.92}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
\toprule
Method   & Type           & Clean          & PGD-50         & C\&W           & AA             & \begin{tabular}[c]{@{}c@{}}Data \\ Memory\end{tabular}   & Time \\ \midrule
FGSM-NR  & Random-based   & 86.41          & 43.99          & 45.4           & 41.29          & \begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}     & 1 $\times$   \\ \midrule
FGSM-RS  & Random-based   & 86.65          & 44.12          & 45.65          & 42.2           & \begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}     & 1  $\times$   \\ \midrule
FGSM-BR  & Random-based   & \textbf{86.82} & 44.23          & 45.89          & 42.37          & \begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}     & 1   $\times$  \\ \midrule
ATTA     & Prior-based    & 86.30          & 44.97          & 43.8           & 42.84          & \begin{tabular}[c]{@{}c@{}}Whole \\ Dataset\end{tabular} & 1   $\times$  \\ \midrule
FGSM-PGI & Prior-based    & 86.61          & 45.69          & 44.8           & 43.26          & \begin{tabular}[c]{@{}c@{}}Whole \\ Dataset\end{tabular} & 1   $\times$  \\ \midrule
FGSM-SDI & Learning-based & 85.25          & \textbf{51.79} & \textbf{50.29} & \textbf{47.91} & \begin{tabular}[c]{@{}c@{}}One \\ Batch\end{tabular}     & 1.6 $\times$  \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/init_v2.tex <==
\begin{table*}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using ResNet18 with different sample initialization techniques. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10_init}
\scalebox{0.82}{
\begin{tabular}{@{}c|c|c|c|c|c|c@{}}
\toprule
Method   & Type           & \begin{tabular}[c]{@{}c@{}}Clean\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-50\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\&W\\ Best/Last\end{tabular} & \begin{tabular}[c]{@{}c@{}}AA\\ Best/Last\end{tabular} & Time \\ \midrule
FGSM-NR  & Random-based   & 84.87/86.41                                               & 45.21/43.99                                                & 45.88/45.4                                               & 41.9/41.29                                             & 1 $\times$  \\ \midrule
FGSM-RS  & Random-based   & 84.91/86.65                                               & 45.43/44.12                                               & 45.66/45.65                                              & 42.77/42.2                                             & 1 $\times$    \\ \midrule
FGSM-BR  & Random-based   & 85.38/\textbf{86.82}                                               & 45.57/44.23                                                & 46.46/45.89                                              & 42.99/42.37                                            & 1 $\times$    \\ \midrule
ATTA     & Prior-based    & 85.97/86.30                                               & 45.97/44.97                                                & 44.6/43.8                                               & 43.39/42.84                                            & 1 $\times$    \\ \midrule
FGSM-PGI & Prior-based    & \textbf{86.33}/86.61                                               & 46.71/45.69                                                & 45.5/44.8                                                & 43.99/43.26                                            & 1 $\times$    \\ \midrule
FGSM-SDI & Learning-based & 84.76/85.25                                               & \textbf{51.79/51.79}                                               & \textbf{51.0/50.29}                                             & \textbf{48.50/47.91}                                           & 1.6 $\times$  \\ \bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table*}

==> table/init_v3.tex <==
\begin{table}[t]
\centering
\caption{ Comparisons of clean and robust accuracy (\%) and training time on the CIFAR-10 database using ResNet18 with different initialization techniques. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10_init}
\scalebox{0.7}{
\begin{tabular}{@{}c|c|c|c|c|c|c@{}}
\toprule
Method   & Type           & \begin{tabular}[c]{@{}c@{}}Clean\end{tabular} & \begin{tabular}[c]{@{}c@{}}PGD-50\end{tabular} & \begin{tabular}[c]{@{}c@{}}C\&W\end{tabular} & \begin{tabular}[c]{@{}c@{}}AA\end{tabular} & Time \\ \midrule
FGSM-NR  & Random-based   & 86.41                                               & 43.99                                                & 45.4                                               &41.29                                             & 1 $\times$  \\ \midrule
FGSM-RS  & Random-based   & 86.65                                               & 44.12                                               & 45.65                                              & 42.2                                             & 1 $\times$    \\ \midrule
FGSM-BR  & Random-based   & \textbf{86.82}                                               & 44.23                                                & 45.89                                              & 42.37                                            & 1 $\times$    \\ \midrule
ATTA     & Prior-based    & 86.30                                               & 44.97                                                & 43.8                                               & 42.84                                            & 1 $\times$    \\ \midrule
FGSM-PGI & Prior-based    & 86.61                                               & 45.69                                                & 44.8                                                & 43.26                                            & 1 $\times$    \\ \midrule
FGSM-SDI & Learning-based & 85.25                                               & \textbf{51.79}                                               & \textbf{50.29}                                             & \textbf{47.91}                                           & 1.6 $\times$  \\ \bottomrule
\end{tabular}
}
\vspace{-4mm}
\end{table}

==> table/reg.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 using ResNet18 with different regularization methods. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10_regularization}
\scalebox{0.54}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
\toprule
Method        & Clean & PGD-10 & PGD-20 & PGD-50 & C\&W  & AA    & Time \\ \midrule \midrule
Baseline    & 86.82 & 46.62  & 44.76  & 44.23  & 45.89 & 42.37  & 1 $\times$    \\ \midrule \midrule
Guided Regularization(min-max)  & 83.33 & 52.04  & 51.03  & 50.96  & 48.64 & 46.56 & $2 \times$   \\ \midrule
Guided Regularization(min)      & 84.20 & 52.38  & 51.54  & 51.26  & 47.87 & 45.74 & $1.4 \times$  \\ \midrule
Nuclear-Norm Regularization(min-max) & 84.9  & 51.21  & 50.09  & 49.79  & 49.14 & 47.36 & $2 \times$   \\ \midrule
Nuclear-Norm Regularization(min)     & \textbf{84.94} & 51.94  & 51.0   & 50.78  & 48.83 & 47.06 & $1.4 \times$ \\ \midrule 
Ours(min)     & 82.97 & \textbf{55.49}  & \textbf{54.58} & \textbf{54.29}  & \textbf{50.41} & \textbf{48.05} & $1.4 \times$ \\ \bottomrule
\end{tabular}}
\end{table}

==> table/wa.tex <==
\begin{table}[t]
\centering
\caption{ Comparisons of clean and robust accuracy (\%) and training time on the CIFAR-10 database using ResNet18 with different model weight averaging techniques under $\ell_{\infty}= 8/225$. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:wa}
\scalebox{0.63}{
\begin{tabular}{@{}c|c|c|c|c|c|c|c@{}}
\toprule
Method      & Clean          & PGD-10         & PGD-20         & PGD-50        & C\&W           & AA    & \begin{tabular}[c]{@{}c@{}}Training\\ Time (min)\end{tabular}      \\ \midrule
Baseline    & 86.82 & 46.62  & 44.76  & 44.23  & 45.89 & 42.37  & 51 \\ \midrule \midrule
Vanilla EMA~\cite{rebuffi2021fixing}  & \textbf{86.91} & 47.1           & 45.64          & 45.1          & 46.53          & 42.8  & 52 \\ \midrule
SE-EMA~\cite{wang2022self}      & 86.82          & 47.42          & 45.71          & 45.26        & 46.68          & 42.92 & 52 \\ \midrule
Auto-EMA(Ours)        & 83.62          & \textbf{51.26} & \textbf{50.21} & \textbf{49.9} & \textbf{49.42} &  \textbf{46.53}     & 52 \\ \bottomrule
\end{tabular}}
\vspace{-2mm}
\end{table}

==> table/wide_cifar10.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using WideResNet34-10 with different adversarial training methods. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10_wide}
\scalebox{0.92}{

\begin{tabular}{@{}c|c|c|c|c|c|c@{}}
\toprule
CIFAR-10  & Clean          & PGD-10         & PGD-20         & PGD-50         & AA             & Time \\ \midrule
PGD-AT    & 85.17          & 56.1           & 55.07          & 54.87          & 51.67          & 5.2 $\times$ \\ \midrule  \midrule
FGSM-RS   & 74.3           & 42.3           & 41.2           & 40.9           & 38.4           & 1 $\times$   \\ \midrule
FGSM-PGI  & 85.09          & 57.72          & 56.86          & 56.4           & 50.11          & 1.4 $\times$ \\ \midrule
FGSM-CKPT & \textbf{91.84} & 44.7           & 42.72          & 42.25          & 40.46          & 1.5 $\times$  \\ \midrule
FGSM-SDI  & 86.4           & 55.89          & 54.95          & 54.6           & 51.17          & 1.6 $\times$ \\ \midrule
NuAT      & 85.30          & 55.8           & 54.68          & 53.75          & 50.06          & 2.0 $\times$ \\ \midrule
GAT       & 85.17          & 56.3           & 55.23          & 54.97          & 50.01          & 2.0 $\times$  \\ \midrule
FGSM-GA   & 82.1           & 48.9           & 47.1           & 46.9           & 45.7           & 3.5 $\times$ \\ \midrule
Free-AT   & 80.1           & 47.9           & 46.7           & 46.3           & 43.9           & 4.2 $\times$ \\ \midrule
Ours      & 84.78          & \textbf{59.88} & \textbf{59.26} & \textbf{59.12} & \textbf{52.29} & 1.4 $\times$ \\ \bottomrule
\end{tabular}
}
\end{table}

==> table/wide_cifar10_v2.tex <==
\begin{table}[t]
\centering
\caption{ Test robustness (\%) on the CIFAR-10 database using WideResNet34-10 with different adversarial training methods. Number in bold indicates the best. 
% Number in bold indicates the best of the fast AT methods. 
}
\label{table:cifar10_wide}
\scalebox{0.92}{

\begin{tabular}{@{}c|c|c|c|c|c|c@{}}
\toprule
CIFAR-10  & Clean          & PGD-10         & PGD-20         & PGD-50         & AA             & Time \\ \midrule
PGD-AT    & 85.17          & 56.1           & 55.07          & 54.87          & 51.67          & 5.2 $\times$ \\ \midrule  \midrule
FGSM-RS   & 74.3           & 42.3           & 41.2           & 40.9           & 38.4           & 1 $\times$   \\ \midrule
FGSM-PGI  & 85.09          & 57.72          & 56.86          & 56.4           & 50.11          & 1.4 $\times$ \\ \midrule
FGSM-CKPT & \textbf{91.84} & 44.7           & 42.72          & 42.25          & 40.46          & 1.5 $\times$  \\ \midrule
FGSM-SDI  & 86.4           & 55.89          & 54.95          & 54.6           & 51.17          & 1.6 $\times$ \\ \midrule
NuAT      & 85.30          & 55.8           & 54.68          & 53.75          & 50.06          & 2.0 $\times$ \\ \midrule
GAT       & 85.17          & 56.3           & 55.23          & 54.97          & 50.01          & 2.0 $\times$  \\ \midrule
FGSM-GA   & 82.1           & 48.9           & 47.1           & 46.9           & 45.7           & 3.5 $\times$ \\ \midrule
Free-AT   & 80.1           & 47.9           & 46.7           & 46.3           & 43.9           & 4.2 $\times$ \\ \midrule
Ours      & 84.78          & \textbf{59.88} & \textbf{59.26} & \textbf{59.12} & \textbf{52.29} & 1.4 $\times$ \\ \bottomrule
\end{tabular}
}
\end{table}
